Probing the theoretical description of central exclusive production

We investigate the theoretical description of the central exclusive production process, $h_1 + h_2 \to h_1+X+h_2$. Taking Higgs production as an example, we compute the subset of next-to-leading order corrections sensitive to the Sudakov factor appearing in the process. Our results agree with those originally presented by Khoze, Martin and Ryskin except that the scale appearing in the Sudakov factor, $\mu=0.62 \sqrt{\hat{s}}$, should be replaced with $\mu=\sqrt{\hat{s}}$, where $\sqrt{\hat{s}}$ is the invariant mass of the centrally produced system. We show that the replacement leads to approximately a factor 2 suppression in the cross-section for central system masses in the range 100--500GeV.

==> Sections/AllOrders.tex <==
\section{All orders Higgs production} \label{sec:CEPAllOrders}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The inclusion of large logarithms appearing at all orders in the perturbation series is crucial if we are to obtain a good approximation to the CEP amplitude. Indeed, as we saw at lowest order, the result is divergent without them\footnote{Actually, the amplitude must be finite even without the inclusion of Sudakov effects, since as $\bs{Q}_\perp \to 0$ the wavelength of the exchanged gluons becomes too large to resolve the colourless protons. Such an effect requires the introduction of hadronic wavefunctions and it has been studied in~\cite{Cudell:2008gv}, using a simple non-perturbative model~\cite{Gunion:1976iy,Levin:1981rf}.}. The logarithmically enhanced terms correspond to emissions that are collinear with external particles and/or soft. In the next sub-section we shall discuss the subset of these corrections corresponding to hard collinear emissions, deferring a treatment of soft emissions to section \ref{sec:softCEPeffects}.


\subsection{Hard collinear emissions}\label{sec:HardCollinear}
%--------------------------------------------------------------------------------------

\subsubsection{Corrections that factorise into the pdfs}\label{sec:pdfs}
%.........................................................................................
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\center
	\includegraphics[width=0.6\textwidth]{FeynmanDiagrams/HardCollinear/Ansatz/Ansatz.epsi}
	\caption{Factorisation of the central exclusive Higgs production amplitude.}\label{fig:Ansatz}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We begin with the ansatz that the central exclusive Higgs production amplitude, $\mathcal{A}_{\textrm{CEP}}$, factorises at some scale, $\mu_F$, much lower than all other scales in the problem. The amplitude may then be written (for small $x_1$ and $x_2$) as
\begin{align}
	\mathcal{A}_{\textrm{CEP}} &\approx 2s\sum_{a_0, \bar{a}_0}\int \! \d\xi_0 \int \! \d\bar{\xi}_0 \; H_{a_0}(\xi_0,\eta;\mu_F^2)H_{\bar{a}_0}(\bar{\xi}_0,\bar{\eta};\mu_F^2) \nonumber \\ 
	& \qquad \qquad \quad \times C^{a_0\bar{a}_0}(\xi_0,\eta,\mu_F^2;\bar{\xi}_0,\bar{\eta},\mu_F^2)~,
\end{align}
where the kinematics are shown in figure~\ref{fig:Ansatz} and we define
\begin{align}
	p^{\mu} &= p_1^{\mu}+p_1'^{\mu} \;,\\
	\bar{p}^{\mu} &= p_2^{\mu} + p_2'^{\mu} \;.
\end{align}
The large logarithmic corrections to the coefficient function, $C^{a_0\bar{a}_0}$, may be computed by cutting off the parton transverse momenta at $\mu_F$, which is equivalent to dimensional regularisation in the $\overline{\textrm{MS}}$ scheme~\cite{Catani:1990rr}. The hard collinear corrections may be organised into two transverse momentum ordered chains as follows:
\begin{align}
	C^{a_0\bar{a}_0}(\xi_0,\eta,\mu_F^2;\bar{\xi}_0,\bar{\eta},\mu_F^2) &= \sum_{n=0}^{\infty} \left[ 
\left(   -\sum_{a_n} \int_{\mu_F^2}^{\bs{Q}_\perp^2} \frac{\d l_n^2}{l_n^2} \frac{\alpha_s(l_n^2)}{4\pi}\int \d\xi_n K_{(0)}^{a_na_{n-1}}  \right)
\right. \nonumber \\
	& \qquad \cdots \left. 
\left(  -\sum_{a_1}\int_{\mu_F^2}^{l_2^2} \frac{\d l_1^2}{l_1^2}\frac{\alpha_s(l_1^2)}{4\pi} \int \d\xi_1 K_{(0)}^{a_1a_0}  \right) 
\right] \nonumber \\
	&\times \sum_{\bar{n}=0}^{\infty} \left[ 
\left(   -\sum_{\bar{a}_{\bar{n}}} \int_{\mu_F^2}^{\bar{\bs{Q}}_\perp^2} \frac{\d \bar{l}_{\bar{n}}^2}{\bar{l}_{\bar{n}}^2}  \frac{\alpha_s(\bar{l}_{\bar{n}}^2)}{4\pi}\int \d\bar{\xi}_{\bar{n}} K_{(0)}^{\bar{a}_{\bar{n}}\bar{a}_{\bar{n}-1}}  \right)
\right. \nonumber \\
	& \qquad \cdots \left. 
\left(  -\sum_{\bar{a}_1}\int_{\mu_F^2}^{\bar{l}_2^2} \frac{\d\bar{l}_1^2}{\bar{l}_1^2}\frac{\alpha_s(\bar{l}_1^2)}{4\pi} \int \d\bar{\xi}_1 K_{(0)}^{\bar{a}_1\bar{a}_0}  \right)
\right] \nonumber \\
	& \otimes C^{a_n\bar{a}_{\bar{n}}}_{\textrm{2 s-channel}}(\xi_n,\eta; \bar{\xi}_{\bar{n}},\bar{\eta}) ~,\label{eq:CollinearChain}
\end{align}
where $\bs{Q}_\perp$ and $\bar{\bs{Q}}_\perp$ are the transverse momenta of the two $s$-channel (``rung'') emissions closest to the hard scatter.  The convolution symbol $\otimes$ indicates that these momenta are integrated over (e.g. see equation~(\ref{eq:c2qq})). 
The $K^{ij}_{(0)}$ are the analogue of the DGLAP splitting functions in the case of skewed kinematics. We have omitted their arguments for clarity but it is to be understood that 
$$K^{a_i a_{i-1}}_{(0)}=K^{a_i a_{i-1}}_{(0)}\left(  \frac{\eta+\xi_{i}}{2},\frac{\eta-\xi_{i}}{2} \Big| \frac{\eta+\xi_{i-1}}{2},\frac{\eta-\xi_{i-1}}{2} \right). $$
They are given by~\cite{Belitsky:2005qn}
\begin{align}
	&K^{qq}_{(0)}(x_1,x_2|y_1,y_2) = C_F \left[  \frac{x_1}{x_1-y_1}\vartheta_{11}^0(x_1,x_1-y_1)+\frac{x_2}{x_2-y_2}\vartheta_{11}^0(x_2,x_2-y_2) \right. \nonumber \\
	& \qquad \qquad \qquad\qquad\qquad\qquad \qquad +\vartheta_{111}^0(x_1,-x_2,x_1-y_1)  \Big]_+  \;,\nonumber\\
	%K^{qg}_{(0)}(x_1,x_2|y_1,y_2) &= -\frac{n_fT_F}{2}\left[  \vartheta_{111}^1(x_1,-x_2,x_1-y_1)\left( 1+\frac{(y_1-x_1)(y_1-x_2)}{y_1y_2}\right) \right. \nonumber\\
	%& \qquad  \qquad \qquad \left. - \vartheta_{111}^0(x_1,-x_2,x_1-y_1)\frac{(x_1-y_1)}{y_1y_2}  \right] \;, \\
	&K^{qg}_{(0)}(x_1,x_2|y_1,y_2) = \frac{T_F}{2} \left[  \vartheta_{112}^1(x_1,-x_2,x_1-y_1)  +2\frac{x_1-y_1}{y_1y_2}\vartheta_{111}^0(x_1,-x_2,x_1-y_1)  \right] \nonumber \\
	&K^{gq}_{(0)}(x_1,x_2|y_1,y_2) = 2C_F \left[  (y_1-y_2)\vartheta_{111}^0(x_1,-x_2,x_1-y_1) \right. \nonumber \\
	 & \quad \qquad\qquad \qquad \qquad \qquad \qquad \qquad \left.+x_1x_2\vartheta_{111}^1(x_1,-x_2,x_1-y_1)  \right] \;, \nonumber \\
	&K^{gg}_{(0)}(x_1,x_2|y_1,y_2) = C_A \left[    \frac{x_1}{y_1}\left[  \frac{x_1}{x_1-y_1}\vartheta_{11}^0(x_1,x_1-y_1) \right]_+ \right. \nonumber \\ 
	&\qquad \quad+ \frac{x_2}{y_2}\left[  \frac{x_2}{x_2-y_2}\vartheta_{11}^0(x_2,x_2-y_2)  \right]_+  +2\frac{x_1x_2+y_1y_2}{y_1y_2}\vartheta_{111}^0(x_1,-x_2,x_1-y_1)\nonumber \\
	&\qquad \quad +2\frac{x_1x_2}{y_1y_2}\frac{x_1y_1+x_2y_2}{(x_1+x_2)^2}\vartheta_{11}^0(x_1,-x_2) +\left(\frac{1}{2}\frac{\beta_0}{C_A}+2  \right)\delta(x_1-y_1) \Big] \; , \label{eq:splittingkernels}
\end{align}
where the generalised step function is defined as
\begin{align}
	\vartheta_{\alpha_1\cdots \alpha_j}^k(x_1,\ldots ,x_j) &= \int \frac{\d\kappa}{2\pi i}\frac{\kappa^k}{\prod_{l=1}^j(x_l \kappa -1 +i \varepsilon)}
\end{align}
and the plus-distribution is given by
\begin{align}
	\left[  \frac{x_1}{x_1-y_1}\vartheta_{11}^0(x_1,x_1-y_1)  \right]_+ &= \frac{x_1}{x_1-y_1}\vartheta_{11}^0(x_1,x_1-y_1) \nonumber \\
	& \quad - \delta(x_1-y_1)\int \d x_1' \frac{x_1'}{x_1'-y_1}\vartheta_{11}^0(x_1',x_1'-y_1) \;.
\end{align}
Note that our definitions of the kernels differ slightly from those of~\cite{Belitsky:2005qn}, in particular:
\begin{align}
	K^{qq}_{(0)} &= K^{qq}_{(0)}|_{\textrm{\cite{Belitsky:2005qn}}} \qquad \qquad K^{qg}_{(0)} = \frac{1}{4 n_f}K^{qg}_{(0)}|_{\textrm{\cite{Belitsky:2005qn}}} \nonumber \\
	K^{gq}_{(0)} &=2 K^{gq}_{(0)}|_{\textrm{\cite{Belitsky:2005qn}}} \qquad \qquad K^{gg}_{(0)} =  K^{gg}_{(0)}|_{\textrm{\cite{Belitsky:2005qn}}} \;.
\end{align}

The collinear logarithms may now be absorbed into the pdfs:
\begin{align}
	\mathcal{A}_{\textrm{CEP}} &\approx 2s \sum_{a,\bar{a}} \int \d\xi \int \d\bar{\xi} \; H_a(\xi,\eta;\bs{Q}_\perp^2) H_{\bar{a}}(\bar{\xi},\bar{\eta};\bar{\bs{Q}}_\perp^2)  \; C^{a\bar{a}}_{\textrm{2 s-channel}}(\xi,\eta; \bar{\xi},\bar{\eta})
\end{align}
where
\begin{align}
	H_a(\xi,\eta;\bs{Q}_\perp^2) &= H_a(\xi,\eta;\mu_F^2) + \sum_{a_0} \int \! \d\xi_0 \; H_{a_0}(\xi_0,\eta;\mu_F^2) \nonumber \\
	& \qquad \times \sum_{n=1}^\infty \left(  -\prod_{j=1}^{n-1} \sum_{a_j} \int_{\mu_F^2}^{l_{j+1}^2}\frac{\d l_j^2}{l_j^2} \frac{\alpha_s(l_j^2)}{4\pi}\int \! \d\xi_j \; K_{(0)}^{a_ja_{j-1}}  \right) \nonumber \\
	& \qquad \times \left(   -\int_{\mu_F^2}^{\bs{Q}_\perp^2} \frac{\d l_n^2}{l_n^2} \frac{\alpha_s(l_n^2)}{4\pi} K_{(0)}^{aa_{n-1}}\left( \frac{\eta+\xi}{2},\frac{\eta-\xi}{2}\Big| \frac{\eta+\xi_{n-1}}{2},\frac{\eta-\xi_{n-1}}{2}  \right)  \right)
\end{align}
and likewise for $H_{\bar{a}}(\bar{\xi},\bar{\eta};\bar{\bs{Q}}_\perp^2)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
	\center
	\subfigure[]{\label{fig:Cqqa}\includegraphics[height=0.35\textwidth]{FeynmanDiagrams/HardCollinear/Cqq/1/1.epsi}} \hspace{0.05\textwidth}
	\subfigure[]{\label{fig:Cqqb}\includegraphics[height=0.35\textwidth]{FeynmanDiagrams/HardCollinear/Cqq/2/2.epsi}}  \\
	\subfigure[]{\includegraphics[height=0.35\textwidth]{FeynmanDiagrams/HardCollinear/Cqq/3/3.epsi}}  \hspace{0.15\textwidth}
	\subfigure[]{\label{fig:Cqqd}\includegraphics[height=0.35\textwidth]{FeynmanDiagrams/HardCollinear/Cqq/4/4.epsi}} 
	\caption{Diagrams contributing to $C^{qq}_{\textrm{2 s-channel}}$.}\label{fig:Cqq}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To study the coefficient function, we take $\{ a,\bar{a}\} = \{  q,q \}$ as an example. The diagrams contributing to $C^{qq}_{\textrm{2 s-channel}}$ are shown in figure~\ref{fig:Cqq}. The contribution from figure~\ref{fig:Cqqa}, for example, may be written
\begin{align}
	&C^{qq}_{\textrm{2 s-channel}}(\xi,\eta;\bar{\xi},\bar{\eta})|_{\textrm{\ref{fig:Cqqa}}} = \nonumber \\
	&\qquad \qquad \times \left(  \frac{i g^2 T_F}{4N} \sum_{a} \int \! \frac{\d^4Q}{(2\pi)^4} \frac{\textrm{Tr}\left[ \gamma^- \gamma^{\mu} \slashed{Q} \gamma^\alpha  \right]}{[Q^2+i\varepsilon][(y_1p-Q)^2+i\varepsilon][(y_2p+Q)^2+i\varepsilon] }\right) \nonumber \\
	&\qquad \qquad   \times \left( \frac{i g^2 T_F}{4N} \sum_{\bar{a}} \int \! \frac{\d^4\bar{Q}}{(2\pi)^4} \frac{\textrm{Tr}\left[ \gamma^+ \gamma^{\nu} \bar{\slashed{Q}} \gamma_\alpha  \right]}{[\bar{Q}^2+i\varepsilon][(\bar{y}_1\bar{p}-\bar{Q})^2+i\varepsilon][(\bar{y}_2\bar{p}+\bar{Q})^2+i\varepsilon]} \right) \nonumber \\
	&\qquad \qquad  \times  \frac{1}{4} i (y_1p-Q)^2 (2\pi)^4 \delta^{(4)}(y_1p+\bar{y}_1\bar{p}-Q-\bar{Q}) V_{H\mu\nu}^{a\bar{a}}(y_2p+Q,\bar{y}_2 \bar{p}+\bar{Q}) ~,
\end{align}
where $y_1 = (\eta+\xi)/2$, $y_2 =(\eta - \xi)/2$ and likewise for $\bar{y}_1,\; \bar{y}_2$. 
The factor of $1/4$ on the third line corrects for double counting after integration over $\xi$ and $\bar{\xi}$. We may approximate the delta-function as
\begin{align}
	\delta^{(4)}(y_1p+\bar{y}_1\bar{p} -Q-\bar{Q}) \approx \delta(y_1 p^+-Q^+)\delta(\bar{y}_1\bar{p}^--\bar{Q}^-) \delta^{(2)}(Q_\perp + \bar{Q}_\perp)~,
\end{align}
which decouples the momentum fraction integrals of the upper and lower sections of the diagram. In addition, if we keep only terms producing a power divergence in $Q_\perp$ and use the gauge invariance of the Higgs vertex, $V_H$, we may make the replacements
\begin{align}
	\textrm{Tr}\left[  \gamma^- \gamma^{\mu} \slashed{Q} \gamma^{\alpha}  \right] &\approx \frac{8}{p^+}(y_2-y_1)\frac{Q^\mu_\perp p^\alpha}{x_1} \;, \\
	\textrm{Tr}\left[  \gamma^+ \gamma^{\nu} \bar{\slashed{Q}} \gamma_\alpha  \right] &\approx \frac{8}{\bar{p}^-}(\bar{y}_2 -\bar{y}_1) \frac{\bar{Q}_\perp^\nu \bar{p}_\alpha}{x_2} \;.
\end{align}
Furthermore, we may write
\begin{align}
	\frac{Q_\perp^{\mu} \bar{Q}_\perp^\nu}{\bs{Q}_\perp^2} V_{H\mu\nu}^{a\bar{a}} &= \bar{V}_H \delta^{a\bar{a}} \nonumber \\
		& = \delta^{a\bar{a}} \frac{1}{2}\frac{1}{N^2-1} \sum_{a_1a_2}\sum_{\epsilon_1 \epsilon_2} \delta^{a_1a_2}\delta_{\epsilon_1 -\epsilon_2} \epsilon_1^\mu \epsilon_2^\nu V_{H\mu\nu}^{a_1a_2}~.
\end{align}
This is the origin of the requirement that the gluons fusing to produce the Higgs have equal helicities, as in equation~(\ref{eq:Mbar}).

Collecting everything together, we have
\begin{align}
	2s \; C^{qq}_{\textrm{2 s-channel}}(\xi,\eta;\bar{\xi},\bar{\eta})|_{\textrm{\ref{fig:Cqqa}}} &\approx \int \! \frac{\d \bs{Q}_\perp^2}{\bs{Q}_\perp^4} \left( -\frac{1}{2} K^{gq}\left( 0,\frac{x_1}{2}\Big| y_1,y_2  \right)  \right) \nonumber \\
	&\qquad \times \left( -\frac{1}{2} K^{gq}\left( 0,\frac{x_2}{2}\Big| \bar{y}_1,\bar{y}_2  \right)  \right)  \nonumber \\
	& \qquad \times \frac{\pi^3 2^2 (-i)}{x_1x_2(N^2-1)} \bar{V}_H \;. \label{eq:c2qq}
\end{align}
Including the other diagrams, \ref{fig:Cqqb}--\ref{fig:Cqqd} and incoming gluons, we find
\begin{align}
	\mathcal{A}_{\textrm{CEP}} &\approx \int \! \frac{\d \bs{Q}_\perp^2}{\bs{Q}_\perp^4} \sum_{a,\bar{a}} \int \d\xi \int \d\bar{\xi} \; H_a(\xi,\eta;\bs{Q}_\perp^2) H_{\bar{a}}(\bar{\xi},\bar{\eta};\bs{Q}_\perp^2) \nonumber \\
	& \times \left( -\frac{1}{2} \tilde{K}^{ga}\left( 0,\frac{x_1}{2}\Big| y_1,y_2  \right)  -\frac{1}{2} \tilde{K}^{ga}\left( \frac{x_1}{2},0\Big| y_1,y_2  \right)  \right) \nonumber \\
	& \times \left( -\frac{1}{2} \tilde{K}^{g\bar{a}}\left( 0,\frac{x_2}{2}\Big| \bar{y}_1,\bar{y}_2  \right)   -\frac{1}{2} \tilde{K}^{g\bar{a}}\left( \frac{x_2}{2},0\Big| \bar{y}_1,\bar{y}_2  \right)  \right) \nonumber \\
	& \times  \frac{\pi^3 2^2 (-i)}{x_1x_2(N^2-1)} \bar{V}_H \;. \label{eq:CEPwithKtilde}
\end{align}
Here, the $\tilde{K}$ denote the unregularised splitting kernels, i.e. the kernels of equations~(\ref{eq:splittingkernels}) but without the plus-prescription. The absence of the plus-prescription is due to a mismatch between the corrections which have the form of a self-energy and those involving the exchange of a parton in the $s$-channel. The mismatch occurs because diagrams, such as the one shown in figure~\ref{fig:PowSuppressed}, not involving at least one $s$-channel parton collinear to each hadron, are suppressed by the centre-of-mass energy. For now, we shall simply replace them with the regularised kernels but this point requires a proper treatment of soft gluon effects, which we shall cover in the next section. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
	\center
	\subfigure[]{\label{fig:PowLeading}\includegraphics[width=0.3\textwidth]{FeynmanDiagrams/HardCollinear/PowerLeading/PowerLeading.epsi}} \hspace{0.03\textwidth}
	\subfigure[]{\label{fig:PowSuppressed}\includegraphics[width=0.3\textwidth]{FeynmanDiagrams/HardCollinear/PowerSuppressed/PowerSuppressed.epsi}}
	\caption{Two diagrams contributing to CEP. The left-hand diagram makes a leading contribution, whereas the right-hand diagram is suppressed by the centre-of-mass energy.}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The pdfs satisfy an evolution equation, analagous to the DGLAP equation in non-skewed kinematics~\cite{Belitsky:2005qn}:
\begin{align}
	\frac{\partial}{\partial\ln \mu_F}\boldsymbol{H}(\xi,\eta;\mu_F^2) &= -\frac{\alpha_s}{2\pi} \int_{-1}^1 \! \d\xi' \; \boldsymbol{K}_{(0)}\left(\frac{\eta+\xi}{2},\frac{\eta-\xi}{2}\Big|\frac{\eta+\xi'}{2},\frac{\eta-\xi'}{2}\right) \boldsymbol{H}(\xi',\eta;\mu_F^2) \;, \label{eq:evolution}
\end{align}
where
\begin{align}
	\boldsymbol{H} &= \left(   \begin{array}{c} H_q \\ H_g  \end{array} \right)
\end{align}
and
\begin{align}
	\boldsymbol{K}_{(0)} &= \left(   \begin{array}{cc} K_{(0)}^{qq} & K_{(0)}^{qg} \\ K_{(0)}^{gq} & K_{(0)}^{gg} \end{array} \right) \;.
\end{align}
We may then use this equation and the symmetry relation, $H_g(-\xi,\eta;\bs{Q}_\perp^2)=H_g(\xi,\eta;\bs{Q}_\perp^2)$~\cite{Belitsky:2005qn}, to write
\begin{align}
	\mathcal{A}_{\textrm{CEP}} &\approx \int \! \frac{\d\bs{Q}_\perp^2}{\bs{Q}_\perp^4}  \frac{\partial}{\partial \ln(\bs{Q}_\perp^2)} \left[ H_g\left(\frac{x_1}{2},\frac{x_1}{2};\bs{Q}_\perp^2\right)\right]  \frac{\partial}{\partial \ln(\bs{Q}_\perp^2)} \left[ H_g\left(\frac{x_2}{2},\frac{x_2}{2};\bs{Q}_\perp^2\right) \right] \nonumber \\
	& \qquad \qquad \qquad \times \frac{\pi^3 2^4 (-i)}{x_1x_2(N^2-1)} \bar{V}_H \;. \label{eq:CEPpdfderiv}
\end{align}


\subsubsection{Corrections that generate the Sudakov factor}\label{sec:suda}
%...............................................................................................................

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
	\center
	\subfigure[]{\label{fig:Sudakova}\includegraphics[width=0.45\textwidth]{ExtraDiagrams/1/1.epsi} \hspace{0.06\textwidth}
	\includegraphics[width=0.35\textwidth]{FeynmanDiagrams/SudakovDiagrams/a/a.epsi}}   \\
	\subfigure[]{\label{fig:Sudakovb}\includegraphics[width=0.35\textwidth]{FeynmanDiagrams/SudakovDiagrams/b/b.epsi}} 
	\caption{Form of large logarithmic corrections to $V_H$ due to emissions collinear to $k_2$.}\label{fig:SudakovDiagrams}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Although we have now dealt with all emissions that factorise into the pdfs, there are still large logarithms contained in $\bar{V}_H$. Again, we deal first with the hard collinear logarithms, deferring the treatment of the soft region to section~\ref{sec:softCEPeffects}.

The diagrams contributing a collinear logarithm with respect to $k_2$ are shown in figure~\ref{fig:SudakovDiagrams}, with equivalent diagrams for $q$ collinear to $k_1$ not shown. Dealing with diagram~\ref{fig:Sudakova} first, we obtain
\begin{align}
	V^{ab}_{H\mu\nu}|_{\textrm{\ref{fig:Sudakova}}} &= \int \! \frac{\d^4q}{(2\pi)^4} \frac{(-i)}{q_1^2+i\varepsilon}\frac{(-i)}{q_2^2+i\varepsilon}f^{cbd}V_{3\alpha\nu\beta}(-q_2,k_2,-q_1) V_\mu'^{\beta\alpha;acd} \;. 
\end{align}
The three-gluon vertex is
\begin{align}
	V_{3\alpha\nu\beta}(-q_2,k_2,-q_1) &= g( g_{\alpha\nu}(-q_2-k_2)_\beta +g_{\nu\beta}(k_2+q_1)_\alpha +g_{\beta\alpha}(q_2-q_1)_\nu ) \nonumber \\
	&\to g (-(1+z_1)g_{\alpha\nu}k_{2\beta} + (1+z_2)g_{\beta\nu}k_{2\alpha})  \nonumber \\
	& \approx g\left(  -\frac{1+z_1}{1-z_1} g_{\alpha\nu} q_{1\beta} +\frac{1+z_2}{1-z_2}g_{\beta\nu}q_{2\alpha} \right)  \label{eq:zPggEikonal}
\end{align}
where we introduced the following Sudakov decomposition of the $q_i$:
\begin{align}
	q_i^{\mu} &= (1-z_i) \hat{k}_2^\mu +\beta_i v^\mu + q_{i\perp} 
\end{align}
with
\begin{align}
	\hat{k}_2^\mu &= k_2^\mu - \frac{k_2^2}{2 k_2 \cdot v} v^\mu\;,  \qquad \quad \hat{k}^2_2 =v^2=0 \;.
\end{align}
In equation~(\ref{eq:zPggEikonal}) we first used the fact that we may set $q_i^{\mu} \approx (1-z_i) k_2^\mu$ in the numerator, up to terms that do not generate a logarithm. Following this, we used the transversality of the incoming gluons to set $k_2^\nu \to 0$. We also multiplied and divided by $1-z_i$. This last step is perfectly valid for hard collinear emissions, however, it will require modification when we come to consider soft effects.

Now observe that $q_{1\beta} V_\mu'^{\beta\alpha;acd}$ and $q_{2\alpha}V_\mu'^{\beta\alpha;acd}$ describe a set of diagrams with an external gluon attached whose polarisation vector is in the direction of its momentum, i.e. it is longitudinally polarised. The QCD Ward identity may then be applied to factor this gluon from $V'$, onto an eikonal line (see for example~\cite{Collins:1989gx}). This is shown in figure~\ref{fig:Sudakova}  and gives the following expression
\begin{equation}
	V_{H\mu\nu}^{ab}|_{\textrm{\ref{fig:Sudakova}}}  = \int \! \frac{\d^4q}{(2\pi)^4} \frac{(-i)}{k_2'^2+i\varepsilon}\frac{(-i)}{q^2+i\varepsilon}f^{cbd}(-gg_{\alpha\nu}(1+z)k_{2\beta} ) \frac{i}{(-q\cdot v)} igv^{\beta}(-if^{dec})V_{H\mu\alpha}^{ae}
\end{equation}
where 
\begin{align}
	q^{\mu}&=(1-z)\hat{k}_2^\mu +\beta v^\mu +q_\perp^\mu \;.
\end{align}
Now, doing the $\beta$ integral by contour integration, we find
\begin{align}
	V_{H\mu\nu}^{ab}|_{\textrm{\ref{fig:Sudakova}}} & \approx - \frac{\alpha_s}{4\pi} C_A \int_0^1 \! \d z \int_{(1-z)z \bs{Q}_\perp^2} \frac{\d l_1^2}{l_1^2} \frac{(1+z)}{1-z} V_{H\mu\nu}^{ab}  \;, \label{eq:wrong}
\end{align}
with $l_1^2 = \bs{q}^2_\perp -(1-z)z k_2^2$ and we made the replacement $k_2^2\approx -\bs{Q}_\perp^2$. Note that, since we are only concerned with the logarithmic terms, we may replace the lower limit on the $l_1^2$ integral as $(1-z)z \bs{Q}_\perp^2 \to (1-z) \bs{Q}_\perp^2$. 

Before discussing the contribution from figure~\ref{fig:Sudakovb}, we note that these logarithmic corrections are going to generate the Sudakov factors, however, observe that the transverse momentum integral extends down to $(1-z)\bs{Q}_\perp^2$. This is in contrast to the integral in the Sudakov factor, which is cut off at $\bs{Q}_\perp^2$, though note that the difference is only relevant for the $(1-z)^{-1}$ term coming from diagram~\ref{fig:Sudakova}. It appears then that, if we cut off the $z$-integral at $1-z \sim |\bs{q}_\perp|/m_H$ (see section~\ref{sec:softCEPeffects}), this piece will generate a Sudakov factor with twice the double logarithmic contribution of equation~(\ref{eq:DurhamSudakov}). This is not the case however. 

Working in the transverse momentum ordered approximation (see equation~(\ref{eq:CollinearChain})), we have missed a contribution from diagrams like those shown in figure~\ref{fig:Nonptordereda} and \ref{fig:Nonptorderedb}. Clearly the diagrams in figure \ref{fig:SudakovDiagrams} cannot account for the screening of long wavelength emissions which results from the colour neutrality of the $t$-channel exchange (since they are oblivious to the role of the screening gluon). Fortunately,
the contribution from diagrams like those of figure~\ref{fig:Nonptordered}, in the region $\bs{q}_\perp^2<\bs{Q}_\perp^2$, with the $(1-z)^{-1}$ piece generating a logarithm, is included in the BFKL corrections. As we shall now see, the BFKL equation guarantees that there is in fact no large logarithm generated by the transverse momentum integral in this region and fixes the lower limit on the $l_1^2$ integral in equation (\ref{eq:wrong}) at $\bs{Q}_\perp^2$ rather than $(1-z)\bs{Q}_\perp^2$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tbh]
	\center
	\subfigure{\label{fig:Nonptordereda}\includegraphics[height=0.25\textwidth]{ExtraDiagrams/2/2.epsi}} \hspace{0.05\textwidth}
	\subfigure{\label{fig:Nonptorderedb}\includegraphics[height=0.25\textwidth]{ExtraDiagrams/3/3.epsi} } 
	\caption{An example of diagrams generating a logarithm not included in the transverse momentum ordered approximation.}\label{fig:Nonptordered}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tbh]
	\center
	\subfigure{\includegraphics[height=0.3\textwidth]{FeynmanDiagrams/BFKLDiagrams/1/1.epsi}} \hspace{0.05\textwidth}
	\subfigure{\includegraphics[height=0.3\textwidth]{FeynmanDiagrams/BFKLDiagrams/2/2.epsi} } \hspace{0.05\textwidth}
	\subfigure{\includegraphics[height=0.3\textwidth]{FeynmanDiagrams/BFKLDiagrams/3/3.epsi} }
	\caption{Next-to-leading order corrections to quark-quark central exclusive production in the BFKL formalism. Slashed gluon propagators and vertices labelled $\Gamma$ indicate reggeised gluons and Lipatov vertices respectively, see~\cite{Forshaw:1997dc}. Not shown are diagrams with the Higgs to the left of the cut.}\label{fig:NLOBFKL}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Consider the one-loop corrections to $C^{qq}$ in the BFKL region, displayed in figure~\ref{fig:NLOBFKL}, where we calculate the amplitude from cuts as described in section~\ref{sec:CEPLO}. In this region, the full set of virtual corrections to either side of the cut
% which include the $|\bs{q}_\perp| \sim |\bs{Q}_\perp|$ piece of $\bar{V}_H$ we have been discussing, 
are summed up in the reggeised gluon propagator (denoted by a slash). These corrections amount to the replacement, in the lowest order graphs, of
\begin{align}
	\frac{1}{Q^2(x_1p_1-Q)^2 (x_2p_2+Q)^2}  &\to \frac{1}{Q^2(x_1p_1-Q)^2 (x_2p_2+Q)^2} \left(\frac{s}{\bs{Q}_\perp^2}  \right)^{2\epsilon_G(Q^2)}~, \label{eq:ReggeReplacement}
\end{align}
where the gluon Regge trajectory, $\epsilon_G(Q^2)$, is given by
\begin{align}
	\epsilon_G(Q^2) &= -\frac{C_A \alpha_s}{(2\pi)^{d-2}} \int \! \d^{d-2}\bs{k}_\perp \frac{\bs{Q}_\perp^2}{\bs{k}_\perp^2(\bs{k}_\perp-\bs{Q}_\perp)^2} \nonumber \\
	& = -\frac{2C_A\alpha_s}{(2\pi)^{d-2}} \int \! \d^{d-2}\bs{k}_\perp \frac{\bs{Q}_\perp^2}{(\bs{k}_\perp-\bs{Q}_\perp)^2[\bs{k}_\perp^2+(\bs{k}_\perp-\bs{Q}_\perp)^2]} \nonumber \\
	& = \frac{C_A\alpha_s}{2\pi}\frac{(4\pi)^\epsilon}{\Gamma(1-\epsilon)} \frac{(\bs{Q}_\perp^2)^{-\epsilon}}{\epsilon} \label{eq:GluonRegge}\;.
\end{align}
%Note that the transverse momentum integral in $\epsilon_G(Q^2)$ only generates a logarithm for $\bs{k}_\perp^2<\bs{Q}_\perp^2$. 
%So as stated, these corrections only include this region of the correction to $\bar{V}_H$. 
Note that there is no double logarithm. Moreover, the region $\bs{k}_\perp^2<\bs{Q}_\perp^2$ generates only single logarithms in $s/\bs{Q}_\perp^2$, i.e. it does not lead to any logarithms in $m_H^2/\bs{Q}_\perp^2$. The complementary region,  $\bs{k}_\perp^2>\bs{Q}_\perp^2$ does not generate a transverse momentum logarithm and as such it is never able to generate a logarithm in the Higgs mass (although it does contribute to a logarithm in $s$, which can be absorbed into the pdfs). Hence we are justified in fixing the infra-red cutoff in equation (\ref{eq:wrong}) equal to $\bs{Q}_\perp^2$.  It will be instructive to observe how the elimination of the would-be double logs and the corresponding gluon reggeisation comes about in section~\ref{sec:FullNLO}, where we present an explicit calculation of the next-to-leading order corrections to $C^{qq}$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb]
	\center
	\includegraphics[height=0.55\textwidth]{FeynmanDiagrams/BFKLDiagrams/4/4.epsi}
	\caption{Schematic form of the central exclusive production amplitude in the BFKL formalism. The functions $f$ are related to the four-gluon Green function and $\Phi$ are proton impact factors, see~\cite{Forshaw:1997dc}.}\label{fig:CEPBFKL}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[b]
	\center
	\subfigure{\includegraphics[height=0.3\textwidth]{FeynmanDiagrams/BFKLDiagrams/5/5.epsi}} \hspace{0.05\textwidth}
	\subfigure{\includegraphics[height=0.3\textwidth]{FeynmanDiagrams/BFKLDiagrams/6/6.epsi} } \hspace{0.05\textwidth}
	\subfigure{\includegraphics[height=0.3\textwidth]{FeynmanDiagrams/BFKLDiagrams/7/7.epsi} }
	\caption{The BFKL integral equation in diagrammatic form.}\label{fig:BFKLequation}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We will close this discussion on BFKL by showing that the would-be infra-red divergence arising from $\epsilon_G(Q^2)$ is cancelled by emissions across the cut, which can be written in terms of the Lipatov vertex, $\Gamma_{\mu\nu}^\sigma$ (see \cite{Forshaw:1997dc} equation~(3.11)). After re-summation, the BFKL corrections can be absorbed into a function, $f(\omega,\bs{k}_\perp,\bs{Q}_\perp)$, which is related to the Green function with four off-shell gluons (see \cite{Forshaw:1997dc} equation~(4.8))\footnote{$\omega$ is a Mellin transform variable, conjugate to the centre-of-mass energy.}. The amplitude may then be computed after convolution with some non-perturbative function containing the long-distance physics associated with the external hadrons, as depicted schematically in figure~\ref{fig:CEPBFKL}.  $f(\omega,\bs{k}_\perp,\bs{Q}_\perp)$ obeys an integral equation, the BFKL equation, shown diagrammatically in figure~\ref{fig:BFKLequation}, i.e.
\begin{align}
	\omega f(\omega,\bs{Q}_\perp,\bs{k}_\perp) &= \delta^{(2)}(\bs{Q}_\perp - \bs{k}_\perp) + \frac{C_A\alpha_s}{\pi^2}\int \! \frac{\d^2\bs{k}_\perp'}{(\bs{k}_\perp'-\bs{Q}_\perp)^2} f(\omega,\bs{k}_\perp',\bs{k}_\perp)  \nonumber \\
	& \qquad +2 \epsilon_G(-\bs{Q}_\perp^2) f(\omega,\bs{Q}_\perp,\bs{k}_\perp) \nonumber \\
	&=  \delta^{(2)}(\bs{Q}_\perp - \bs{k}_\perp)  \nonumber \\
	& \qquad +\frac{C_A \alpha_s}{\pi^2} \int \! \frac{\d^2\bs{k}_\perp'}{(\bs{k}_\perp'-\bs{Q}_\perp)^2} \left(  f(\omega,\bs{k}_\perp',\bs{k}_\perp)  - \frac{\bs{Q}_\perp^2 f(\omega,\bs{Q}_\perp,\bs{k}_\perp)}{[\bs{k}_\perp'^2 + (\bs{k}_\perp'-\bs{Q}_\perp)^2]}  \right)~.
\end{align}
Now observe that, for $\bs{k}_\perp'^2 \ll \bs{Q}_\perp^2$, the first and second terms in parenthesis (the first term corresponds to emissions across the cut) cancel one another. 

The above is essentially the same argument, though presented in slightly different terms, that the Durham group use to set the lower limit on the Sudakov factor in equation~(\ref{eq:BFKLTrick}). We will verify this argument explicitly in section~\ref{sec:FullNLO}, where we detail the results of a full next-to-leading order calculation of the virtual corrections which contribute to the Sudakov factor.

Returning to the calculation of diagram~\ref{fig:Sudakova}, we find
\begin{align}
	V_{H\mu\nu}^{ab}|_{\textrm{\ref{fig:Sudakova}}} & \approx - \frac{\alpha_s}{4\pi} C_A \int_0^1 \! \d z \int_{\bs{Q}_\perp^2}^{l_2^2} \frac{\d l_1^2}{l_1^2} \frac{(1+z)}{1-z} V_{H\mu\nu}^{ab}  \;.
\end{align}
In addition to replacing the lower limit, we have now made explicit the upper limit of the $l_1^2$ integration. The variable $l_2$ is the analogue of $l_1$, but for the next emission contained in $V_H$. 

Next, the one-loop gluon propagator corrections (see for example~\cite{Grozin:2007zz}) give, for figure~\ref{fig:Sudakovb},
\begin{align}
	V_{H\mu\nu}^{ab}|_{\textrm{\ref{fig:Sudakovb}}} & \approx \frac{\alpha_s}{4\pi} \left( \frac{10}{12}C_A - \frac{2 T_F n_f}{3}  \right) \int_{-k_2^2}^{\mu_R^2} \! \frac{\d l_1^2}{l_1^2} V_{H\mu\nu}^{ab}~,
\end{align}
where $\mu_R$ is the renormalisation scale. By setting $\mu_R^2=l_2^2$, the two contributions in figure~\ref{fig:SudakovDiagrams} may be rewritten in terms of the DGLAP splitting functions, with the additional effect that the strong coupling now runs with $l_1^2$:
\begin{align}
	\bar{V}_H|_{n\textrm{ collinear emissions}} &= -2 \int^{l_2^2}_{\bs{Q}_\perp^2} \frac{\d l_1^2}{l_1^2} \frac{\alpha_s(l_1^2)}{4\pi} \int_0^1 \d z \left(  z \tilde{P}_{gg}(z) +n_f P_{qg}(z) \right) \nonumber \\
	& \qquad \qquad \qquad \qquad  \times  \bar{V}_H|_{n-1\textrm{ collinear emissions}}\label{eq:VHcollinear}
\end{align}
and we also included the contribution from emissions collinear to $k_1$. The tilde again denotes the splitting function without the plus-prescription.

Equation~(\ref{eq:VHcollinear}) is still incorrect as it stands, since the integral diverges in the soft limit, $z \to 1$. This is an artifact of our hard collinear approximation: for fixed, finite, transverse momentum, a soft gluon's energy cannot vanish. We shall discuss how this problem is rectified in the next section. For now, we ignore the divergence and iterate (\ref{eq:VHcollinear}) until we are left with the tree level vertex:
\begin{align}
	\bar{V}_H &= \sum_{n=0}^{\infty} \prod_{i=1}^n \left(   - \int_{\bs{Q}_\perp^2}^{l_{i+1}^2}  \frac{\d l_i^2}{l_i^2} \frac{\alpha_s(l_i^2)}{4\pi} \int_0^1 \d z \left( z\tilde{P}_{gg}(z) +n_f P_{qg}(z)  \right)  \right) \nonumber \\
	& \quad \times \sum_{\bar{n}=0}^{\infty} \prod_{\bar{i}=1}^{\bar{n}} \left(   - \int_{\bs{Q}_\perp^2}^{\bar{l}_{\bar{i}+1}^2} \frac{\d\bar{l}_{\bar{i}}^2}{\bar{l}_{\bar{i}}^2} \frac{\alpha_s(\bar{l}_{\bar{i}}^2)}{4\pi} \int_0^1 \d z \left( z\tilde{P}_{gg}(z) +n_f P_{qg}(z)  \right)  \right) \nonumber \\
	& \quad \times \overline{\mathcal{M}}(gg \to H)~, \label{eq:VHemissions}
\end{align}
where $l_{n+1}^2=\bar{l}_{\bar{n}+1}^2 =m_H^2$ and $\overline{\mathcal{M}}$ is as defined in equation~(\ref{eq:Mbar}). We may then use the following identity for ordered integrals
\begin{align}
	\int_{\bs{Q}_\perp^2}^{l_2^2} \d l_1^2 \cdots \int_{\bs{Q}_\perp^2}^{m_H^2} \d l_n^2 &= \frac{1}{n!}\prod_{j=1}^n \int_{\bs{Q}_\perp^2}^{m_H^2} \d l_j^2
\end{align}
which allows us to rewrite equation~(\ref{eq:VHemissions}) in terms of exponentials:
\begin{align}
	\bar{V}_H &= \exp \left[  -\int_{\bs{Q}_\perp^2}^{m_H^2} \frac{\d l^2}{l^2} \frac{\alpha_s(l^2)}{4\pi} \int_0^1 \d z \left(  z \tilde{P}_{gg}(z) +n_f P_{qg}(z)  \right) \right] \nonumber \\
	& \quad \times  \exp \left[  -\int_{\bs{Q}_\perp^2}^{m_H^2} \frac{\d \bar{l}^2}{\bar{l}^2} \frac{\alpha_s(\bar{l}^2)}{4\pi} \int_0^1 \d z \left(  z \tilde{P}_{gg}(z) +n_f P_{qg}(z)  \right) \right] \nonumber \\
	& \quad \times \overline{\mathcal{M}}(gg \to H) \;. \label{eq:divergentSudakov}
\end{align}
Thus we begin to see the emergence of the Sudakov factors.


\subsection{Soft emissions} \label{sec:softCEPeffects}
%--------------------------------
So far we have deferred the treatment of soft gluon effects: In section \ref{sec:pdfs} we noted that the final rung before the hard scatter involved an unregulated splitting function, e.g. see equation (\ref{eq:CEPwithKtilde}) and in section \ref{sec:suda} we noted a potential divergence in the $z \to 1$ limit of the Sudakov factor, e.g. see equation (\ref{eq:VHemissions}). We shall now turn our attention to these matters and consider the soft gluon limit more carefully than hitherto.

\subsubsection{The Sudakov factor}
%..............................................................

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
	\center
	\includegraphics[width=0.35\textwidth]{FeynmanDiagrams/SoftEffects/1/1.epsi}
	\caption{Form of the softest gluon attachment to the Higgs vertex.}\label{fig:softHiggsvertex}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We shall begin our discussion of soft effects by dealing with the $z \to 1$ divergence in the Higgs vertex corrections. The softest gluon must attach to both gluons fusing to produce the Higgs, as shown in figure~\ref{fig:softHiggsvertex}. This contribution has the form
\begin{align}
	\bar{V}_H|_{n\textrm{ soft emissions}} &= \frac{i C_A g^2 m_H^2}{(2\pi)^4} \int \! \d^2 q_{\perp} \int \! \d \alpha \int \! \d\beta \nonumber \\
	& \qquad \qquad \qquad \times \frac{\bar{V}_H|_{n-1\textrm{ soft emissions}}}{[q^2+i\varepsilon][(q-k_1)^2+i\varepsilon][(q+k_2)^2+i\varepsilon]} \label{eq:VHsoft1}
\end{align}
where
\begin{align}
	q^\mu &= \alpha k_1^\mu + \beta k_2^\mu + q_\perp^\mu \;. \label{eq:qSudakovDecomp}
\end{align}
This diagram contains divergences both when $q$ is collinear to $k_1$ and when it is collinear to $k_2$. In order to bring the result into the form of equation~(\ref{eq:VHcollinear}) we must separate out these two regions. An effective way to accomplish this is to multiply the integrand of~(\ref{eq:VHsoft1}) by
\begin{align}
	1 &= \textrm{PV}\left( \frac{\alpha}{\alpha+\beta}  \right) +\textrm{PV}\left( \frac{\beta}{\alpha+\beta}  \right)
\end{align}
where PV denotes the Cauchy principal value. Now the term proportional to $\alpha/(\alpha+\beta)$ possesses only a collinear divergence with respect to $k_1$, whereas the other piece has only a collinear divergence when $q \propto k_2$. We may then perform the $\beta(\alpha)$ integrals in the first(second) term by contour integration. Only the piece coming from the $[q^2+i\varepsilon]$ pole is relevant to the $(1-z)^{-1}$ divergence. Keeping just this piece, we obtain
\begin{align}
	\bar{V}_H|_{n\textrm{ soft emissions} }&= -\frac{\alpha_s}{2\pi} C_A \int \! \frac{\d\bs{q}_\perp^2}{\bs{q}_\perp^2} \left(  \int_0^1 \! \d\alpha \frac{1}{\alpha +\frac{\bs{q}_\perp^2}{\alpha m_H^2}}  +  \int_0^1 \! \d|\beta| \frac{1}{|\beta| +\frac{\bs{q}_\perp^2}{|\beta| m_H^2}}  \right) \nonumber \\
	& \qquad \qquad \qquad \times \bar{V}_H|_{n-1\textrm{ soft emissions}}~.
\end{align}
Changing variables as $\alpha = 1-z$, $|\beta| = 1-z$ and noting that the momentum fraction integrals are effectively cutoff at $|\bs{q}_\perp|/m_H$, this becomes
\begin{align}
	\bar{V}_H|_{n\textrm{ soft emissions}} &= - 2 \frac{\alpha_s}{2\pi} C_A \int \! \frac{\d\bs{q}_\perp^2}{\bs{q}_\perp^2} \int_0^{1-|\bs{q}_{\perp}|/m_H} \frac{\d z}{1-z}\bar{V}_H|_{n-1\textrm{ soft emissions}}
\end{align}
and so equation~(\ref{eq:divergentSudakov}) becomes
\begin{equation}
	\bar{V}_H = T(\bs{Q}_\perp,m_H) \overline{\mathcal{M}}(gg \to H) ~,
\end{equation}
with
\begin{equation}
T(\bs{Q}_\perp,m_H) =
\exp \left(  -\int_{\bs{Q}_\perp^2}^{m_H^2} \frac{\d\bs{q}_\perp^2}{\bs{q}_\perp^2} \frac{\alpha_s(\bs{q}_\perp^2)}{2\pi} \int_0^{1-|\bs{q}_{\perp}|/m_H} \d z \left[  z P_{gg}(z) +n_f P_{qg}(z)  \right] \right)~. \label{eq:MyAllOrdersSudakov}
\end{equation}
Note that this result differs from equations (\ref{eq:DurhamSudakov})--(\ref{eq:DurhamMU}). In sections~\ref{sec:FullNLO} and \ref{sec:NLO2} we shall provide further evidence that equation (\ref{eq:MyAllOrdersSudakov}) is indeed the correct form of the Sudakov factor.

\subsubsection{The Sudakov derivative}
%.....................................................................

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[b]
	\centering
	\subfigure[]{\label{fig:SudDeriv1}\includegraphics[width=0.4\textwidth]{FeynmanDiagrams/SoftEffects/2/2.epsi}} \hspace{0.05\textwidth}
	\subfigure[]{\label{fig:SudDeriv2}\includegraphics[width=0.4\textwidth]{FeynmanDiagrams/SoftEffects/3/3.epsi}}
	\caption{Diagrams for the last emission collinear to the upper hadron which generate the soft part of the splitting kernel.}\label{fig:SudDeriv}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now turn our attention to a proper treatment of the (unregularised) splitting kernels entering due to the final two $s$-channel emissions. The only issue is with the $K^{gg}$ kernel, which diverges in the soft limit. In order to understand how to treat this region correctly we focus on the final emission collinear to the upper hadron, assuming all previous emissions have been collected into the pdf. 

As discussed in section~\ref{sec:CEPLO}, we may compute the amplitude by taking the cuts shown in figures~\ref{fig:CEPgeneralcuts1} and \ref{fig:CEPgeneralcuts5} only. Furthermore, if we wish to study the soft limit of the final emission, only the diagrams shown in figure~\ref{fig:SudDeriv} and the analogous diagrams with the Higgs emitted on the other side of the cut will contribute. In addition, we need only consider the sub-set of these diagrams in which $Q$ attaches to on-shell particles. The result is then given by the soft insertion rules (see for example~\cite{Bassetto:1984ik}). After summing the two diagrams in figure~\ref{fig:SudDeriv}, for example, the amplitude to the left of the cut, $\ket{L_1}^{\mu,a}$, may be written
\begin{align}
	\ket{L_1}^{\mu,a} &= \sum_{i=0}^{n+1} \left(  \frac{-g l_i^{\mu}}{l_i\cdot Q} \right) \bs{T}^a_{l_i} \ket{L_0}~,
\end{align}
where $l_0 = y_1 p$, $l_{n+1}=\bar{y}_2 \bar{p}$ and the other $l_i$ are the momenta of the particles crossing the cut. The amplitude without the soft gluon is represented by $\ket{L_0}$. Since $Q$ is the last emission collinear to the upper proton, we may take $l_i \propto \bar{p}$ for $i \neq 0$. Including the amplitude to the right of the cut, $\ket{R_1}$, using the same soft insertion formula and including an integration over the intermediate phase-space,  we obtain
\begin{align}
	A|_{\textrm{\ref{fig:SudDeriv}}} &= -\int \! \d(PS^n) \int \! \frac{\d^4 Q}{(2\pi)^3} \delta_{(+)}(Q^2) \frac{g^2 \; p\cdot \bar{p}}{p\cdot Q \; \bar{p} \cdot Q} \nonumber \\
	& \qquad \times \sum_{i=1}^{n+1} \left(   \bra{R_0}(\bs{T}_{l_i}^a)^\dagger \bs{T}_{l_0}^a \ket{L_0} +\bra{R_0}(\bs{T}_{l_0}^a)^\dagger \bs{T}_{l_i}^a \ket{L_0} \right)~,
\end{align}
where $\d(PS^n)$ is the phase-space of the cut diagram without the soft gluon. Then, using colour conservation:
\begin{align}
	\sum_{i=1}^{n+1} \bs{T}_{l_i}^a &= - \bs{T}^a_{l_0} \;, \\
	(\bs{T}_{l_0}^a)^\dagger \bs{T}_{l_0}^a &= C_A \;,
\end{align}
we find
\begin{align}
	A|_{\textrm{\ref{fig:SudDeriv}}} &= \int \! \d(PS^n) \int \! \frac{\d^4 Q}{(2\pi)^3} \delta_{(+)}(Q^2) \frac{C_A g^2 \; p\cdot \bar{p}}{p \cdot Q \; \bar{p} \cdot Q} 2 \braket{R_0|L_0} \;. \label{eq:SudDerivSoft1}
\end{align}
Now note that (\ref{eq:SudDerivSoft1}) possesses divergences when $Q$ becomes collinear to either $p$ or $\bar{p}$. As in the case of the Sudakov factor, we may separate out these regions by multiplying the integrand by $1=(\alpha+\beta)/(\alpha+\beta)$, where this time
\begin{align}
	Q^\mu &= \alpha p^\mu + \beta \bar{p}^\mu + Q_\perp^\mu \;.
\end{align}
Since we are interested in the divergences with respect to the upper hadron, we keep only the $\alpha/(\alpha+\beta)$ piece. The only effect of the phase-space on $Q$ is to introduce the constraint $\Theta(y_1 p^+ -Q^+)$. Thus, (\ref{eq:SudDerivSoft1}) becomes
\begin{align}
	A|_{\textrm{\ref{fig:SudDeriv}}} &= \frac{2 g^2 C_A}{(2\pi)^3} \int \! \frac{\d^2 \bs{Q}_\perp}{\bs{Q}_\perp^2} \int_0^{y_1} \! \d\alpha \frac{1}{\alpha + \frac{\bs{Q}_\perp^2}{4\alpha s}} \int \! \d(PS^n) \braket{R_0|L_0} \;.
\end{align}
Comparing this to equation~(\ref{eq:splittingkernels}), by taking the limit $x_i \to y_i$, we see that the correct form of the unregularised splitting kernel is
\begin{align}
	\tilde{K}^{gg}_{(0)}(x_1,x_2|y_1,y_2) &= C_A  \left[  \frac{x_1}{y_1}  \frac{x_1 \; \vartheta_{11}^0(x_1,x_1-y_1) }{\left(x_1-y_1+\frac{\bs{Q}_\perp^2}{(x_1-y_1)4s}\right)} \right. \nonumber \\
	& \quad \quad \qquad+ \frac{x_2}{y_2}  \frac{x_2 \; \vartheta_{11}^0(x_2,x_2-y_2)}{\left( x_2-y_2+\frac{\bs{Q}_\perp^2}{(x_2-y_2)4s}\right)}    \nonumber \\
	& \quad \quad \qquad+2\frac{x_1x_2+y_1y_2}{y_1y_2}\vartheta_{111}^0(x_1,-x_2,x_1-y_1) \nonumber \\
	& \quad \quad \qquad +2\frac{x_1x_2}{y_1y_2}\frac{x_1y_1+x_2y_2}{(x_1+x_2)^2}\vartheta_{11}^0(x_1,-x_2) \Bigg] \;.\label{eq:trueUnregKgg}
\end{align}
To the soft divergent pieces we may now add and subtract a term proportional to a delta-function:
\begin{align}
	\frac{x}{y} \frac{x\; \vartheta_{11}^0(x,x-y)}{\left( x-y+\frac{\bs{Q}_\perp^2}{(x-y)4s}\right)} &= \frac{x}{y}\left[ \frac{x \; \vartheta_{11}^0(x,x-y)}{\left( x-y+\frac{\bs{Q}_\perp^2}{(x-y)4s}\right)} \right. \nonumber \\
	& \qquad \quad \left. - \delta(x-y) \int \! \d x' \frac{x'\vartheta_{11}^0(x',x'-y)}{\left( x'-y+\frac{\bs{Q}_\perp^2}{(x'-y)4s}\right)} \right] \nonumber \\
	& \qquad \quad + \delta(x-y) \int \! \d x' \frac{x'\vartheta_{11}^0(x',x'-y)}{\left( x'-y+\frac{\bs{Q}_\perp^2}{(x'-y)4s}\right)} \;.
\end{align}
In the first term, contained in square brackets, we may take the $\bs{Q}_\perp \to 0$ limit since the soft region cancels, leaving us with something regularised by the plus-prescription. The integral in the second term may be done explicitly, giving a logarithm plus non-logarithmic terms which we neglect. Substituting this identity into equation~(\ref{eq:trueUnregKgg}) it becomes
\begin{align}
	\tilde{K}^{gg}(x_1,x_2|y_1,y_2) &= K^{gg}(x_1,x_2|y_1,y_2) - \frac{\alpha_s}{4\pi} C_A \delta(x_1-y_1) \ln \left(  \frac{4y_1^2s+\bs{Q}_\perp^2}{\bs{Q}_\perp^2}  \right) \nonumber \\
	& \quad - \frac{\alpha_s}{4\pi} C_A \delta(x_2-y_2) \ln \left(  \frac{4y_2^2s+\bs{Q}_\perp^2}{\bs{Q}_\perp^2}  \right) \;.
\end{align}
Applying this to the splitting kernels appearing in equation~(\ref{eq:CEPwithKtilde}) gives, e.g.
\begin{align}
	\tilde{K}^{ga}\left( \frac{x_1}{2},0 \Big| y_1,y_2 \right) &= K^{ga}\left( \frac{x_1}{2},0 \Big| y_1,y_2 \right) - \delta^{ga} \frac{\alpha_s}{2\pi} C_A \delta \left(  \xi - \frac{x_1}{2} \right) \ln\left( \frac{m_H^2}{\bs{Q}_\perp^2}  \right)~,
\end{align}
where we replaced $x_1^2 s \to m_H^2$, which is correct to logarithmic accuracy. This logarithm in the Higgs mass may then be written in terms of the derivative of the Sudakov factor:
\begin{align}
	\tilde{K}^{ga}\left( \frac{x_1}{2},0 \Big| y_1,y_2 \right) &= K^{ga}\left( \frac{x_1}{2},0 \Big| y_1,y_2 \right) \nonumber \\
	& \qquad  - \delta^{ga} \delta \left(  \xi - \frac{x_1}{2} \right) \frac{2}{\sqrt{T(\bs{Q}_\perp,m_H)}} \frac{ \partial \sqrt{T(\bs{Q}_\perp,m_H)}}{\partial \ln(\bs{Q}_\perp^2)} \;.
\end{align}
All together then, including the Sudakov factor, equation~(\ref{eq:CEPpdfderiv}) becomes
\begin{align}
	\mathcal{A}_{\textrm{CEP}} &\approx  \int \! \frac{\d\bs{Q}_\perp^2}{\bs{Q}_\perp^4}  \frac{\partial}{\partial \ln(\bs{Q}_\perp^2)} \left[ H_g\left(\frac{x_1}{2},\frac{x_1}{2};\bs{Q}_\perp^2\right) \sqrt{T(\bs{Q}_\perp,m_H)} \right] \nonumber \\
	& \quad \times \frac{\partial}{\partial \ln(\bs{Q}_\perp^2)}  \left[ H_g\left(\frac{x_2}{2},\frac{x_2}{2};\bs{Q}_\perp^2\right) \sqrt{T(\bs{Q}_\perp,m_H)} \right]  \nonumber \\
	& \quad \times \frac{\pi^3 2^4 (-i)}{x_1x_2(N^2-1)} \overline{\mathcal{M}}(gg \to H)  \;.
\end{align}
Finally, using equation~(\ref{eq:RgDeff}) and assuming that $R_g$ depends only weakly on $\bs{Q}_\perp^2$, we find
\begin{align}
	\mathcal{A}_{\textrm{CEP}} &\approx  \int \! \frac{\d\bs{Q}_\perp^2}{\bs{Q}_\perp^4}  f_g(x_1,0,\bs{Q}_\perp^2,m_H^2) f_g(x_2,0,\bs{Q}_\perp^2,m_H^2)  \nonumber \\
	& \qquad \qquad \times \frac{\pi^3 2^4 (-i)}{x_1x_2(N^2-1)} \overline{\mathcal{M}}(gg \to H)  \;.
\end{align}





==> Sections/LowestOrder.tex <==
\section{Lowest order Higgs production}\label{sec:CEPLO}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We begin our investigation of the Durham model by computing (in Feynman gauge) the lowest order amplitude for two quarks of different flavour to scatter into two quarks and a Higgs, $A_{\textrm{LO}}$. We take the quarks as scattering in the forward direction:
\begin{align}
	p_1'^{\mu} &= (1-x_1) p_1^{\mu} \;,\\
	p_2'^{\mu} &= (1-x_2) p_2^{\mu} \;.
\end{align}
The dependence of the amplitude on the outgoing hadron transverse momenta in equation~(\ref{eq:Durhamdsig}) is a non-perturbative effect and so we do not expect to be sensitive to it here. We will also make frequent use of the high energy limit: keeping only terms not suppressed by an inverse power of the centre-of-mass energy. In this limit, there are four lowest order diagrams which contribute, as shown in figure~\ref{fig:LO}. In addition, we work in the effective theory in which the top quark has been integrated out~\cite{Shifman:1979eb,Voloshin:1985tc,Ellis:1975ap}. This generates a point-like coupling of the Higgs to gluons (see appendix~\ref{app:largetop}).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb]
\center
\subfigure[]{\label{fig:LOa}\includegraphics[width=0.35\textwidth]{FeynmanDiagrams/CEP/LowestOrderLabeled/a/a.epsi}} \hspace{0.05\textwidth}
\subfigure[]{\label{fig:LOb}\includegraphics[width=0.35\textwidth]{FeynmanDiagrams/CEP/LowestOrderLabeled/b/b.epsi}} \\
\subfigure[]{\label{fig:LOc}\includegraphics[width=0.35\textwidth]{FeynmanDiagrams/CEP/LowestOrderLabeled/c/c.epsi}}  \hspace{0.05\textwidth}
\subfigure[]{\label{fig:LOd}\includegraphics[width=0.35\textwidth]{FeynmanDiagrams/CEP/LowestOrderLabeled/d/d.epsi}}
\caption{The lowest order diagrams contributing to $q+q'\to q\oplus H \oplus q'$, in the high energy limit.}\label{fig:LO}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For small $x_i$ the amplitude is dominated by the region in which the exchanged gluons are soft and we may therefore take the gluons as coupling to the quark lines via eikonal vertices. Thus, for example, the contribution to the amplitude of graph~\ref{fig:LOa}, with the colour singlet contribution projected out, takes the form
\begin{align}
	A^{\ref{fig:LOa}} &= - i \delta_{\sigma_1\sigma_1'} \delta_{\sigma_2\sigma_2'}16 T_F^2 \frac{N^2-1}{N^2} g^4 p_1 \cdot p_2 \int \! \frac{\d^4Q}{(2\pi)^4} \frac{p_1^{\mu}p_2^{\nu} H_{\mu\nu}(k_1,k_2;\mu)}{\mathcal{D}}~, \label{eq:amp1a}
\end{align}
where
\begin{align}
	\mathcal{D}^{-1} &= [Q^2+i\varepsilon][(Q-p_1)^2+i\varepsilon][(Q+p_2)^2+i\varepsilon] \nonumber \\
			& \quad \times[(Q-x_1p_1)^2+i\varepsilon][(Q+x_2p_2)^2+i\varepsilon]
\end{align}
and the Higgs vertex factor, $H^{\mu\nu}$, has the form (see appendix~\ref{app:largetop})
%and the kinematics are shown in figure~\ref{fig:LOa-labeled}. The Higgs vertex factor, $H^{\mu\nu}$, has the form:
\begin{equation}
	H^{\mu\nu}(k_1,k_2;\mu) = -iC^R_1(\mu)(k_1\cdot k_2 \; g^{\mu\nu} - k_2^{\mu}k_1^{\nu}) \;.
\end{equation}
Working in the centre-of-mass frame of $p_1$ and $p_2$, with $p_1$ defining the $z$-axis, we may evaluate the $Q^+$ and $Q^-$ integrals for each graph. To leading power in the high-energy limit we obtain
\begin{align}
	A^{\ref{fig:LOa}} &= A^{\ref{fig:LOc}} = A^{\ref{fig:LOd}} = 0 \nonumber \\
	A_{\textrm{LO}} &= A^{\ref{fig:LOb}} = A_0(\mu) \int_{\Lambda} \! \frac{\d\boldsymbol{Q}^2_\perp}{\boldsymbol{Q}_\perp^4}~, \label{eq:amps-abcd}
\end{align} 
where $\Lambda$ is a cutoff imposed to define the integral and
\begin{align}
	A_0(\mu) &=  - \delta_{\sigma_1\sigma_1'}\delta_{\sigma_2\sigma_2'}C^R_1(\mu) g^4 \frac{s}{\pi} \frac{T_F^2 C_F}{N} \;.
\end{align}

Some comments are in order at this point. The first is that the amplitude is infrared power-divergent as $\Lambda \to 0$; this is to be expected, since we are dealing with a fixed-order expansion of a parton-level matrix element. As we shall see, this divergence will ultimately be tamed by a Sudakov factor (see also the footnote at the beginning of section~\ref{sec:HardCollinear}). The second comment is that the contribution to the S-matrix ($iA$) is pure imaginary. This is expected for colour singlet exchange in the high energy limit, based on arguments from Regge theory~\cite{Forshaw:1997dc}. Thirdly, note that it is perhaps not surprising that diagram \ref{fig:LOb} gives a different result from all of the other diagrams, since it is the only one in which $Q$ is pinched in the Glauber/Coulomb region~\cite{Bodwin:1981fv,Collins:1981ta}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[b]
	\center
	\subfigure[]{\label{fig:CEPgeneralcuts1}\includegraphics[width=0.25\textwidth]{FeynmanDiagrams/CEPgeneralcuts/Cut1/Cut1.epsi}}
	\subfigure[]{\label{fig:CEPgeneralcuts2}\includegraphics[width=0.25\textwidth]{FeynmanDiagrams/CEPgeneralcuts/Cut2/Cut2.epsi}}
	\subfigure[]{\label{fig:CEPgeneralcuts3}\includegraphics[width=0.25\textwidth]{FeynmanDiagrams/CEPgeneralcuts/Cut3/Cut3.epsi}} \\
	\subfigure[]{\label{fig:CEPgeneralcuts4}\includegraphics[width=0.25\textwidth]{FeynmanDiagrams/CEPgeneralcuts/Cut4/Cut4.epsi}}	
	\subfigure[]{\label{fig:CEPgeneralcuts5}\includegraphics[width=0.25\textwidth]{FeynmanDiagrams/CEPgeneralcuts/Cut5/Cut5.epsi}}
	\caption{The allowed cuts of the CEP amplitude.}\label{fig:CEPgeneralcuts}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Since its imaginary part dominates, we could equally well have used the Cutkosky rules~\cite{Cutkosky:1960sp} to evaluate the amplitude. In fact, it is this approach we shall use to evaluate the next-to-leading order corrections in section~\ref{sec:FullNLO}. The structure of the lowest order calculation will give us some hint as to how we may simplify the next-to-leading order corrections and so we detail it here.


Recall that the Cutkosky rules implement the unitarity relation, which states that if we sum over the cuts of a graph, $G_C$, this sum is proportional to the imaginary part of the graph without the cut, $G$:
\begin{align}
  \sum_C G_C &= 2 \Im {\mathrm{m}} (-i G) \;.\label{eq:Cutkosky}
\end{align}
For a cut to be allowed it must satisfy two conditions: the invariant-mass of the four-momenta on each side of the cut and the total energy flowing from left to right across the cut must both be positive. Given these conditions, the possible cuts of the general CEP amplitude are shown in figure~\ref{fig:CEPgeneralcuts} and the possible cuts of the lowest order diagrams are shown in figure~\ref{fig:LOcuts}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\center
\subfigure[]{\label{fig:LOcut1}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/1.epsi}}\hspace{0.2cm}
\subfigure[]{\label{fig:LOcut2}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/2.epsi}}\hspace{0.2cm}
\subfigure[]{\label{fig:LOcut3}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/3.epsi}}\hspace{0.2cm}
\subfigure[]{\label{fig:LOcut4}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/4.epsi}} \\
\subfigure[]{\label{fig:LOcut5}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/5.epsi}}\hspace{0.2cm}
\subfigure[]{\label{fig:LOcut6}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/6.epsi}}\hspace{0.2cm}
\subfigure[]{\label{fig:LOcut7}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/7.epsi}}\hspace{0.2cm}
\subfigure[]{\label{fig:LOcut8}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/8.epsi}} \\
\subfigure[]{\label{fig:LOcut9}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/9.epsi}}\hspace{0.2cm}
\subfigure[]{\label{fig:LOcut10}\includegraphics[width=0.2\textwidth]{FeynmanDiagrams/CEP/LowestOrder/Cuts/10.epsi}}
 \caption{The possible cuts of the lowest order diagrams.}\label{fig:LOcuts}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



However, it turns out that we need only consider the cuts~\ref{fig:LOcut1} and \ref{fig:LOcut5}; the remaining cuts all cancel amongst one another. The reason for this is that these diagrams represent a sum over soft gluon insertions onto the upper or lower quark lines. The fact that the soft gluon in all these cases is cut ensures that it is not in the Coulomb/Glauber region and we may therefore apply the soft approximation~\cite{Collins:1985ue,Collins:1988ig,Collins:1981ta,Collins:1981uk}. The result is that we may rewrite each sum of diagrams contributing to a given cut as a single diagram with the soft gluon connected to an eikonal line. This is shown explicitly in figure~\ref{fig:CEPsoftapprox} for the diagrams~\ref{fig:LOcut2} and \ref{fig:LOcut7} (see for example~\cite{Collins:1989gx} for the eikonal Feynman rules). The two diagrams differ only in the attachments of the gluons to the upper quark lines, which give the following expressions
\begin{align}
	A^{\textrm{\ref{fig:LOcut2}}} &\propto \frac{t^bt^a}{(p_1-Q)^2}p_1^\mu p_1^\alpha \approx -\frac{t^bt^a}{2p_1 \cdot Q} p_1^\mu p_1^\alpha \\
	A^{\textrm{\ref{fig:LOcut7}}} & \propto \frac{t^at^b}{(p_1'+Q)^2}p_1^\mu p_1^\alpha \approx +\frac{t^at^b}{2p_1 \cdot Q} p_1^\mu p_1^\alpha
\end{align}
Here we took both gluons as soft, dropping all terms suppressed by $Q$ or $x_1$, which allowed us to make the eikonal approximation in the numerator and to set $p_1'\approx p_1$ in the denominator of the second diagram. In addition, the on-shell delta-function gives $|Q^2| =|2x_1p_1\cdot Q| \ll |2p_1 \cdot Q|$, allowing us to approximate the denominators as shown. The sum of diagrams is proportional to the commutator $[t^a,t^b]$ or, put another way, in the eikonal diagram of figure~\ref{fig:CEPsoftapprox} the upper quark line is connected to the lower part of the diagram by a single gluon. The key point is that we are dealing with colour singlet exchange and such diagrams contribute only to the octet exchange part of the amplitude. We may therefore neglect them.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
	\center
	\subfigure{\includegraphics[height=0.25\textwidth]{FeynmanDiagrams/CEPsoftapprox/1/1.epsi}} \hspace{0.005\textwidth}
	\subfigure{\includegraphics[height=0.25\textwidth]{FeynmanDiagrams/CEPsoftapprox/2/2.epsi} } \hspace{0.005\textwidth}
	\subfigure{\includegraphics[height=0.35\textwidth]{FeynmanDiagrams/CEPsoftapprox/3/3temp.epsi} }
	\caption{Rewriting a sum of cuts in terms of an insertion onto an eikonal line.}\label{fig:CEPsoftapprox}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


This situation generalises to all orders and so we need never consider the cuts~\ref{fig:CEPgeneralcuts2}--\ref{fig:CEPgeneralcuts4} since they do not make a leading contribution to the colour singlet exchange amplitude.




==> Sections/Recalculation.tex <==
\section{A further cross-check}\label{sec:NLO2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



We now discuss a re-calculation of the soft part of the Sudakov factor, which exploits the Bloch-Nordsieck theorem~\cite{Bloch:1937pw}. It serves as a further check on our earlier results. In particular, we infer the virtual corrections by considering the set of real emission diagrams making up the $gg\to gH$ amplitude, as shown in figure~\ref{fig:RyskinDiagrams}. The relevant cross-section is given by
\begin{align}
	\sigma &= \int \! \d\xi_1 \int \! \d\xi_2 \; g(\xi_1;\mu_F^2) g(\xi_2;\mu_F^2) \; \frac{1}{2\hat{s}} \frac{\hat{s}}{2} \int \! \d\alpha \int \! \d\beta \int \! \frac{\d^2q_\perp}{(2\pi)^3} \; \delta_{(+)}(q^2) \nonumber \\
	& \qquad \qquad \times (2\pi) \delta_{(+)}((k_1+k_2-q)^2 - m_H^2) |\mathcal{M}|^2
\end{align}
where the $\xi_i$ denote the momentum fractions of the incoming gluons and we parametrise the final-state gluon momentum, $q$, in terms of Sudakov variables as in equation~(\ref{eq:qSudakovDecomp}), with
\begin{align}
	\hat{s} &= 2k_1\cdot k_2  \; .
\end{align}	
The amplitude, $\mathcal{M}$, is summed over equal incoming helicities by contraction with a polarisation vector (in the $k_1$-$k_2$ centre-of-mass frame), $e^\mu = (0,\cos \phi, \sin \phi,0)$ for the incoming gluons, followed by an average over $\phi$ i.e.
\begin{align}
	\mathcal{M} &= \int_0^{2\pi}\frac{d \phi}{2\pi} e^\mu e^\nu \mathcal{M}_{\mu\nu} \;.
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tbp]
	\center
	\subfigure[]{\label{fig:Ryskin1}\includegraphics[height=0.2\textwidth]{FeynmanDiagrams/RyskinDiagrams/1/1.epsi}}  \hspace{0.01\textwidth}
	\subfigure[]{\label{fig:Ryskin2}\includegraphics[height=0.2\textwidth]{FeynmanDiagrams/RyskinDiagrams/2/2.epsi}}  \hspace{0.01\textwidth}
	\subfigure[]{\label{fig:Ryskin3}\includegraphics[height=0.2\textwidth]{FeynmanDiagrams/RyskinDiagrams/3/3.epsi}}  \\
	\subfigure[]{\label{fig:Ryskin4}\includegraphics[height=0.2\textwidth]{FeynmanDiagrams/RyskinDiagrams/4/4.epsi}}   
	\caption{Diagrams contributing to the process $gg\to Hg$.} \label{fig:RyskinDiagrams}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, we divide the phase-space of the emitted gluon into the regions $\alpha>\beta$ and $\alpha<\beta$, which is equivalent to dividing the phase-space about zero rapidity. We shall calculate only the contribution from the $\alpha>\beta$ region, however it will be clear that the $\alpha<\beta$ region gives an equal result. In addition, we sum over final state polarisations using\footnote{Note that, in processes involving two or more external gluons, the replacement of the gluon polarisation sum with $-g^{\mu\nu}$ is not in general valid~\cite{Cutler:1977qm}.}
\begin{align}
	\sum_\lambda \varepsilon_\lambda^\rho(k) \varepsilon^{*\rho'}_\lambda(k) &= -g^{\rho\rho'} + \frac{k_1^\rho k^{\rho'} + k_1^{\rho'}k^{\rho}}{k_1\cdot k} \;.
\end{align}
We also average over incoming gluon colours, though we stress that changing the treatment of colour in the process affects only the normalisation, since each diagram has identical colour structure. After a little algebra, which is performed using FORM, we find
\begin{align}
	\sigma|_{\alpha>\beta} &=   \int \! \d\xi_1 \int \! \d\xi_2 \; g(\xi_1;\mu_F^2) g(\xi_2;\mu_F^2) \frac{1}{2\hat{s}}   \int \! \frac{\d^2 q_\perp}{(2\pi)^2}  \int_{\frac{q_\perp}{\sqrt{\hat{s}}}}^1 \d\alpha  \; |\mathcal{M}^{\textrm{LO}}|^2 \;  C_A \; g^2 \nonumber \\ 
	& \quad \times \delta_{(+)}((k_1+k_2-q)^2-m_H^2) \left\{   \frac{1}{q_\perp^2}\left[ -4 +\frac{2}{\alpha} +4\alpha -2 \alpha^2 +\frac{\alpha^3}{2}  \right]  \right. \nonumber \\ 
	& \quad+ \frac{2}{\hat{s}}\left[  -3 +\frac{4}{\alpha} -\frac{2}{\alpha^2} +\alpha   \right]   + \frac{ q_\perp^2}{\hat{s}^2} \left[  \frac{3}{\alpha} - \frac{6}{\alpha^2} +\frac{4}{\alpha^3}  \right] \nonumber \\  
	& \left. \quad+ \frac{2q_\perp^4}{\hat{s}^3}\left[  \frac{1}{\alpha^3}-\frac{1}{\alpha^4} \right]   + \frac{ q_\perp^6}{2\hat{s}^4} \frac{1}{\alpha^5}  \right\}	  
\end{align}
where
\begin{align}
	\mathcal{M}^{\textrm{LO}} &= \int_0^{2\pi} \frac{\d\phi}{2\pi} e^\mu e^\nu \mathcal{M}^{\textrm{LO}}_{\mu\nu}
\end{align}
is the lowest order $gg\to H$ amplitude summed over equal incoming helicities. The key point to note is that only the term proportional to $1/q_\perp^2$ can generate a logarithm or a constant after the $\alpha$ integral: The remaining terms are insufficiently singular in the soft ($\alpha \to 0$) limit.  Keeping only this term then, changing variables as $\alpha =1-z$, approximating the delta-function and including the region $\alpha<\beta$, we find
\begin{align}
	\sigma &=  \int \! \d\xi_1 \int \! \d\xi_2 \; g(\xi_1;\mu_F^2) g(\xi_2;\mu_F^2) \frac{1}{2\hat{s}}   \int \! \frac{\d q_\perp^2}{q_\perp^2}  \int^{1-\frac{q_\perp}{m_H}}_0 \d z   \nonumber \\
	& \quad \times  (2\pi)\delta_{(+)}(z \hat{s}-m_H^2) |\mathcal{M}^{\textrm{LO}}|^2 \frac{\alpha_s}{\pi}\left(  z P_{gg}(z)  + \frac{C_A}{2}( 3z^3-5z^2+5z-3) )   \right) \;, \label{eq:JeffsRyskinResult}
\end{align}
where we replaced $\sqrt{\hat{s}} \to m_H$ in the upper limit of the $z$ integral, as appropriate in the soft limit. The additional $z$-dependent piece, not proportional to $P_{gg}(z)$, arises due to the restricted sum over incoming helicities and it vanishes in the soft $z \to 1$ limit.\footnote{If we had summed over all incoming helicity configurations this term would of course have been absent.}
Thus, in the soft limit, we find
\begin{align}
	\sigma|_{\textrm{soft}} \propto \int \! \frac{\d q_\perp^2}{q_\perp^2} \frac{C_A \alpha_s}{\pi} \ln \left(  \frac{m_H}{q_\perp} \right) ~,
\end{align}
which further supports the validity of equation~(\ref{eq:MyAllOrdersSudakov}).

